A Bayesian Non-parametric Approach for Causal Mediation with a Post-treatment Confounder

We propose a new Bayesian non-parametric (BNP) method for estimating the causal effects of mediation in the presence of a post-treatment confounder. We specify an enriched Dirichlet process mixture (EDPM) to model the joint distribution of the observed data (outcome, mediator, post-treatment confounders, treatment, and baseline confounders). The proposed BNP model allows more confounder-based clusters than clusters for the outcome and mediator. For identifiability, we use the extended version of the standard sequential ignorability as introduced in \citet{hong2022posttreatment}. The observed data model and causal identification assumptions enable us to estimate and identify the causal effects of mediation, $i.e.$, the natural direct effects (NDE), and indirect effects (NIE). We conduct simulation studies to assess the performance of our proposed method. Furthermore, we apply this approach to evaluate the causal mediation effect in the Rural LITE trial, demonstrating its practical utility in real-world scenarios. \keywords{Causal inference; Enriched Dirichlet process mixture model.}

==> figure/figureEDP_CEstandard.tex <==
\begin{figure}[htbp] %[p]
    \centering
        \begin{tikzpicture}
            [
                rect/.style={minimum size=30pt,rectangle,draw},
                circ/.style={minimum size=30pt,circle,draw},
                thickarro/.style={->,>=stealth',semithick},
                arro/.style={->,>=stealth',},
                dottarro/.style={->,>=stealth',dotted},
            ]
            
            \node (Z) [circ] at (-4.5,0) {$Z$};
            \node (Y) [circ] at (4.5,0) {$Y$};
            
            \node (M) [circ] at (0,1.5) {$M$};
            \node (C) [circ] at (0,-1.5) {$\boldsymbol{C}$};
            
            \draw[thickarro] (Z) -- (Y) node at (1.5,0.2) {};
            \draw[thickarro] (Z) -- (M) node at (-2.5,1) {};
            \draw[thickarro] (M) -- (Y) node at (2.5,1) {};
            \draw[dottarro] (C) -- (M) node at (0.2,0.45) {};
            \draw[dottarro] (C) -- (Y) node at (2.5,-1) {};
            % \draw[thickarro] (Z) -- (Y) node at (1.5,0.2) {a};
            % \draw[thickarro] (Z) -- (M) node at (-2.5,1) {b};
            % \draw[thickarro] (M) -- (Y) node at (2.5,1) {c};
            % \draw[dottarro] (C) -- (M) node at (0.2,0.45) {d};
            % \draw[dottarro] (C) -- (Y) node at (2.5,-1) {e};
        \end{tikzpicture}
        \caption{\label{EDPM.ce.std} The causal structure without a post-treatment confounder and a randomized treatment.}
\end{figure}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> table/tableEDP_real_avg_supp1.tex <==
\begin{table}[htbp]
    % \fontsize{9}{11}\selectfont
    \centering
    \caption{\label{EDPM:tab:avgsupp1} Posterior means (95\% credible intervals) of NIE, NDE, and ATE under the proposed BNP model. $\rho$ is a sensitivity parameter for a post-treatment confounder.}
    \begin{tabular}[htbp]{c|rrr|rrr|rrr}
        \toprule
        \multicolumn{1}{c}{ } & \multicolumn{3}{c}{$\rho \sim \mtri{-1,0,-1}$} & \multicolumn{3}{c}{$\rho \sim \munif{0,1}$} & \multicolumn{3}{c}{$\rho = -0.5 $} \\
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
        CE & Est. & \multicolumn{2}{c}{95\% CI} & Est. & \multicolumn{2}{c}{95\% CI} & Est. & \multicolumn{2}{c}{95\% CI} \\
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
        NIE & -0.88 & -1.46 & -0.34 & -0.37 & -0.88 & 0.12 & -0.80 & -1.30 & -0.26 \\
        NDE & -2.43 & -3.95 & -0.97 & -2.95 & -4.36 & -1.54 & -2.51 & -3.97 & -1.09 \\
        ATE & -3.31 & -4.73 & -1.94 & -3.32 & -4.74 & -1.94 & -3.31 & -4.76 & -1.94 \\
        
        \midrule
        \multicolumn{1}{c}{} & \multicolumn{3}{c}{$\rho = -0.3 $} & \multicolumn{3}{c}{$\rho = 0.3$(true)} & \multicolumn{3}{c}{$\rho = 0.8$} \\
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
        CE & Est. & \multicolumn{2}{c}{95\% CI} & Est. & \multicolumn{2}{c}{95\% CI} & Est. & \multicolumn{2}{c}{95\% CI} \\
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
        NIE & -0.72 & -1.19 & -0.25 & -0.49 & -0.90 & -0.04 & -0.23 & -0.65 & 0.16 \\
        NDE & -2.59 & -4.03 & -1.17 & -2.84 & -4.29 & -1.52 & -3.08 & -4.51 & -1.74 \\
        ATE & -3.31 & -4.77 & -1.83 & -3.33 & -4.83 & -1.98 & -3.31 & -4.77 & -1.92 \\
        \bottomrule
    \end{tabular}
\end{table}

==> table/tableEDP_real_avg_supp2.tex <==
\begin{table}[htbp] %[p]
    % \fontsize{11}{11}\selectfont
    \caption{\label{EDPM:tab:avgsupp2} Posterior means (95\% credible intervals) of NIE, NDE, and ATE under the standard ignorability assumption without a post-treatment confounder.}
    \centering
        \begin{tabular}[htp]{c|rrr} %[htbp]
        \toprule
        \multicolumn{1}{c}{CE} & \multicolumn{1}{c}{Est.} & \multicolumn{2}{c}{95\% CI} \\
        
        \midrule
        NIE & -0.09 & -0.66 &  0.37 \\
        NDE & -3.08 & -4.83 & -1.49 \\
        ATE & -3.17 & -4.83 & -1.61 \\
        \bottomrule

    \end{tabular}
\end{table}
